SGHateCheck: Functional Tests for Detecting Hate Speech in Low-Resource Languages of Singapore

To address the limitations of current hate speech detection models, we introduce \textsf{SGHateCheck}, a novel framework designed for the linguistic and cultural context of Singapore and Southeast Asia. It extends the functional testing approach of HateCheck and MHC, employing large language models for translation and paraphrasing into Singapore's main languages, and refining these with native annotators. \textsf{SGHateCheck} reveals critical flaws in state-of-the-art models, highlighting their inadequacy in sensitive content moderation. This work aims to foster the development of more effective hate speech detection tools for diverse linguistic environments, particularly for Singapore and Southeast Asia contexts.

==> content/app_label_table.tex <==
\label{app:label_table}

Results of hate and non-hate results between models fine-tuned with EngSet and MultiSet can be found in Table \ref{tab:label_results}.

% NO LONGER DISPLAYED
% \begin{table*}[]
%     \small
%     \centering
%     {
%     \begin{tabular}{>{\arraybackslash}m{2cm}*{10}{R}}
%        \toprule
%        \multirow{2}{2cm}{Fine-tune Dataset}
%         & \multicolumn{2}{c}{Average}
%         & \multicolumn{2}{c}{Singlish}
%         & \multicolumn{2}{c}{Malay}
%         & \multicolumn{2}{c}{Mandarin)}
%         & \multicolumn{2}{c}{Tamil}
        
%         \\\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
        
%         & {non-hate} & {hate}
%         & {non-hate} & {hate}
%         & {non-hate} & {hate}
%         & {non-hate} & {hate}
%         & {non-hate} & {hate} \\

%         \midrule
%         EngSet & 0.981 & 0.107 & 0.952 & 0.277 & 0.991
%         & 0.087 & 0.996 & 0.058 & 0.986 & 0.008
%         \\
%         MultiSet & 0.783 & 0.411 & 0.842 & 0.454 & 0.705
%         & 0.502 & 0.624 & 0.627 & 0.961 & 0.058 
%         \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Accuracy for cases labeled non-hate and hate. Average (Avg.) is the average of accuracy for languages}
%     \label{tab:label_results}
% \end{table*}

==> content/app_machine_generation.tex <==
\label{appendix:machine_generation}

To aid with the translations task, translators were shown five fully formed options which they can choose as their final input. They have the choice to choose any (can be more than one) of the options, or choose none of the options and type in their custom text. For each test case or templates to be translated, annotators were shown five options to choose from. 

Details of the sources used for prompt generation is shown below. 

\begin{itemize}
    \item Fine tuned GPT-3.5 \cite{NEURIPS2020_1457c0d6}: GPT-3.5 was fine tuned with Unalignment \cite{gpt3_redteaming} fine tuning dataset in order to jailbreak GPT-3.5's safety behaviour. English test case or template from HateCheck was input as a prompt into the fine tuned GPT-3.5 model.
    \item GPT-4 \cite{gpt4}: English test case or template from HateCheck was input as a prompt into GPT-4. If the response was considered invalid, the prompt was then sent to Fine tuned GPT 3.5. 
    \item Google Cloud Translate: English test case from HateCheck or templates was input as a prompts into Google's Cloud Translation API \cite{google_cloud_translate}.
    \item English sample: Due to the similarity with Singlish, the English test case or template from HateCheck was offered as an option for Singlish translators
\end{itemize}

Instructions for fine tuned GPT-3.5 and GPT-4 were handcrafted with casual social media use in mind. Experimented with the use of personas, a well known method to improve response quality \cite{gpt_personas}. Translators were first shown the outputs to a set of prompts and asked which were preferred. As necessary, this process was iterated for a couple more times until a satisfactory result was achieved. 

For each language, sources are carefully chosen to ensure high quality output can be captured. The choice of source for each language, as well as quantity and prompts are found in Table ~\ref{tab:template_generation_prompts}. The order of the 5 options are randomised when displayed to the translators.

\begin{table*}[]
\begin{tabular}{cc>{\centering\arraybackslash}m{3cm}>{\arraybackslash}m{9cm}}
\toprule
Language                  & \# Options & Source                                                                  & GPT Instructions                                                                                                                                                                                                                                                                                                                  \\
\hline\multirow{2}{*}{Singlish} & 1           & English original                                                        &                                                                                                                                                                                                                                                                                                                             \\
                          \cdashline{2-4} & 4           & Fine tuned GPT-3.5                                                                 & You will be provided with statements, and your task is to convert them to Singlish. Do not include punctuation and there is no need to explain any words. Focus on changing the structure of the sentence to make it more Singlish, instead of just adding words.                                                           \\
\hline\multirow{2}{*}{Malay}    & 1           & Google Translate                                                        &                                                                                                                                                                                                                                                                                                                             \\
                          \cdashline{2-4} & 4           & Fine tuned GPT-3.5                             & Assume that you are a Malay based in Singapore and above is an English template. Tell me one Malay colloquial equivalent to this. Assume a social context. Find expressions which have a similar meaning instead of translating directly.                                                                                   \\
\hline\multirow{3}{*}{Tamil}    & 1           & Google Translate                                                        &                                                                                                                                                                                                                                                                                                                             \\
                          \cdashline{2-4} & 2           & GPT-4& Imagine you are a social media user writing in peecu Tamil, a colloquial form of Tamil used when people speak to each other. Please write the sentence in peecu Tamil, be careful to ensure that the words used in the sentence matches the mood and meaning of the original input sentence. Please output in Tamil script. \\
                          \cdashline{2-4} & 2           & GPT-4 & Imagine you are a social media user writing in peecu Tamil, a colloquial form of Tamil. Rewrite the input text so that it is in an informal, spoken colloquial style. You can do so by including contractions, omissions, or more relaxed word choices.   \\
\bottomrule

\end{tabular}
\caption{Sources of options displayed to translators for selection. Number of options (# Options) represent how many options from the particular source is shown to the translator.}
\label{tab:template_generation_prompts}
\end{table*}

==> content/app_protected_groups.tex <==
\label{appendix:protected_groups}

Protected groups and target identifier for all Singlish, Malay, Mandarin and Tamil datasets can be found in Table \ref{tab:target_placeholders}.

\begin{table*}[]
\begin{adjustwidth}{-4em}{-4em}
\small
\centering
\begin{tabular}{*{2}{>{\arraybackslash}m{2cm}}|>{\centering\arraybackslash}m{1cm}>{\tiny\centering\arraybackslash}m{2cm}>{\centering\arraybackslash}m{2cm}>{\tiny\centering\arraybackslash}m{2cm}}
\toprule
Prt. Grp.                   & Target              & Singlish       & {\small Mandarin } & Malay                    & {\small Tamil}                   \\ \hline
Age                         & Seniors             & seniors        & 老人                                  & orang tua                & {\tam மூத்தவர்}                  \\ \hline
\multirow{2}{*}{Disability} & Mentally ill        & mentally ill   & 精神病患者                               & orang berpenyakit mental & {\tam மனநலம் பாதிக்கப்பட்ட நபர்} \\
                            & Physically Disabled & handicap       & 残疾人                                 & orang kurang upaya       & {\tam உடல் ஊனமுற்றவர்}           \\ \hline
\multirow{3}{*}{Gender}     & Homosexual          & gay            & 同性恋                                 & Orang gay                & {\tam ஓரினச்சேர்க்கையாளர்}       \\
                            & Transsexual         & trans          & 跨性别者                                & orang trans              & {\tam திருநங்கை}                 \\
                            & Women               & woman          & 女人                                  & Perempuan                & {\tam பெண்}                      \\ \hline
Origin                      & Immigrants          & foreign worker & 外国人                                 & Pendatang                & {\tam புலம்பெயர்ந்தவர்}          \\ \hline
\multirow{3}{*}{Race}       & Chinese             & Chinese        & 华人                                  & Cina                     & {\tam சீனர்}                     \\
                            & Indians             & Indian         & 印度人                                 & India                    & {\tam இந்தியன்}                  \\
                            & Malay               & Malay          & 马来人                                 & Melayu                   & {\tam மலாய்}                     \\ \hline
\multirow{4}{*}{Religion}   & Buddhist            & Buddhist       & 佛教徒                                 & Orang buddha             & {\tam பௌத்தன்}                   \\
                            & Christian           & Christian      & 基督徒                                 & Orang Kristian           & {\tam கிறித்துவர்}               \\
                            & Hindu               & Hindu          & 兴都督徒                                & Orang Hindu              & {\tam இந்து}                     \\
                            & Muslim              & Muslim         & 回教徒                                 & Orang Islam              & {\tam இஸ்லாமியர்}                \\
\bottomrule
\end{tabular}
\caption{ Placeholders in Singlish, Mandarin, Malay and Tamil that are used to represent targets in templates. Also shown are the protected groups (Prt. Grp.) that each target belongs to}
\label{tab:target_placeholders}
\end{adjustwidth}
\end{table*}

==> content/discussion.tex <==
% The experiments showed us several ways hate speech detection can be improved.

% First, the use of a strong model is necessary to prevent false negatives for hateful cases. Our experiment showed that weaker models like the SEA-LLM tend to label test cases as non-hate regardless of the case. In real life situations, this means that hate speech can go undetected. 

% Second, a simple way to improve a LLM based model is to finetune the model using LORA of localised dataset. This will partially mitigate the false negative bias (although it will show up as lower accuracy for non-hateful examples due to reduced bias). This method also works if the language here, finetuning dataset is not the same as the test dataset, as seen in the improvements of the Singlish score. 

% Third, comparison of HateCheck, MHC with \textsf{SGHateCheck} suggests that models perform differently for localised and non-localised dataset, even though the localised dataset was largely based on the non-localised dataset. The performance difference suggets non-localised benchmarking has a use in today's world. 

The experiments provide several insights. First of all, we find that Mistral 7B performas better on all checklists across languages except for the two cases, F18 and F22. Mistral 7B performs better than some of the bigger models such as LLaMA2 13B on various NLP tasks. This could explain overall better performance of Mistral 7B. The two cases are an interesting find and need further investigation.

% THIS FILE IS NO LONGER LINKED PLEASE SEE RESULTS DISCUSSION

==> content/functional_tests.tex <==
\begin{table*}
\small
\begin{tabular}{ll*{20}{R}}
\toprule
                       &             & \multicolumn{5}{c}{Singlish Accuracy}        & \multicolumn{5}{c}{Malay Accuracy}           & \multicolumn{5}{c}{Mandarin Accuracy}        & \multicolumn{5}{c}{Tamil Accuracy}            \\ \cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22}
F\#                    & Gold Label  & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM \\
\hline
F1                     & hateful     & 0.326  & 0.246 & 0.681   & 0.014    & 0.601  & 0.608  & 0.24  & 0.576   & 0.120     & 0.872  & 0.892  & 0.446 & 0.992   & 0.057    & 0.928  & 0.000      & 0.022 & 0.037   & 0.000        & 0.000      \\
F2                     & hateful     & 0.398  & 0.096 & 0.831   & 0.000    & 0.771  & 0.620  & 0.463 & 0.639   & 0.046    & 0.954  & 0.794  & 0.431 & 1.000   & 0.157    & 0.971  & 0.000  & 0.056  & 0.112   & 0.000    & 0.000  \\
F3                     & hateful     & 0.427  & 0.183 & 0.779   & 0.000    & 0.740  & 0.508  & 0.308 & 0.523   & 0.015    & 0.954  & 0.877  & 0.352 & 0.984   & 0.074    & 0.926  & 0.000  & 0.056  & 0.126   & 0.000    & 0.000  \\
F4                     & hateful     & 0.492  & 0.150 & 0.734   & 0.017    & 0.671  & 0.507  & 0.271 & 0.243   & 0.100    & 0.650  & 0.566  & 0.184 & 0.846   & 0.279    & 0.640  & 0.000  & 0.056  & 0.175   & 0.000    & 0.040  \\
F4                     & hateful     & 0.519  & 0.130 & 0.878   & 0.000    & 0.702  & 0.470  & 0.289 & 0.417   & 0.104    & 0.922  & 0.755  & 0.230 & 0.942   & 0.137    & 0.921  & 0.000  & 0.057  & 0.100   & 0.000    & 0.000  \\
F5                     & hateful     & 0.703  & 0.464 & 0.964   & 0.007    & 0.935  & 0.647  & 0.489 & 0.619   & 0.079    & 0.978  & 0.829  & 0.464 & 0.950   & 0.214    & 0.929  & 0.000  & 0.131  & 0.238   & 0.000    & 0.000  \\
F7                     & hateful     & 0.600  & 0.000 & 0.500   & 0.000    & 0.500  & 0.556  & 0.556 & 0.333   & 0.000    & 0.778  & 1.000  & 0.400 & 0.800   & 0.000    & 0.600  & 0.000  & 0.100  & 0.000   & 0.000    & 0.000  \\
F8                     & hateful     & 0.579  & 0.214 & 0.793   & 0.007    & 0.779  & 0.629  & 0.500 & 0.536   & 0.064    & 0.886  & 0.928  & 0.667 & 1.000   & 0.232    & 0.877  & 0.000  & 0.044  & 0.106   & 0.000    & 0.000  \\
F9                     & non-hateful & 0.889  & 1.000 & 1.000   & 1.000    & 1.000  & 0.400  & 0.700 & 1.000   & 1.000    & 0.800  & 0.500  & 0.700 & 0.800   & 0.800    & 0.800  & 1.000  & 1.000  & 1.000   & 1.000    & 1.000  \\
F10                    & hateful     & 0.561  & 0.216 & 0.827   & 0.079    & 0.791  & 0.529  & 0.336 & 0.471   & 0.121    & 0.914  & 0.882  & 0.529 & 1.000   & 0.206    & 0.860  & 0.000  & 0.029  & 0.279   & 0.000    & 0.019  \\
F11                    & hateful     & 0.529  & 0.436 & 0.821   & 0.043    & 0.793  & 0.657  & 0.686 & 0.757   & 0.064    & 0.957  & 0.914  & 0.396 & 1.000   & 0.295    & 0.986  & 0.000  & 0.251  & 0.464   & 0.000    & 0.005  \\
F12                    & hateful     & 0.414  & 0.081 & 0.901   & 0.018    & 0.784  & 0.421  & 0.325 & 0.526   & 0.070    & 0.807  & 0.799  & 0.302 & 0.986   & 0.122    & 0.906  & 0.000  & 0.088  & 0.250   & 0.000    & 0.000  \\
F13                    & non-hateful & 0.871  & 0.823 & 0.895   & 0.992    & 0.887  & 0.608  & 0.672 & 0.856   & 0.904    & 0.688  & 0.555  & 0.609 & 0.609   & 0.875    & 0.703  & 1.000  & 0.934  & 0.766   & 1.000    & 0.993  \\
F14                    & hateful     & 0.574  & 0.156 & 0.803   & 0.049    & 0.787  & 0.677  & 0.339 & 0.710   & 0.097    & 0.992  & 0.835  & 0.729 & 1.000   & 0.256    & 0.970  & 0.000  & 0.152  & 0.296   & 0.000    & 0.000  \\
F15                    & hateful     & 0.722  & 0.357 & 0.930   & 0.087    & 0.957  & 0.703  & 0.461 & 0.578   & 0.070    & 0.992  & 0.949  & 0.594 & 0.993   & 0.130    & 0.971  & 0.000  & 0.052  & 0.156   & 0.000    & 0.000  \\
F16                    & non-hateful & 0.984  & 1.000 & 0.992   & 0.984    & 0.992  & 0.748  & 0.901 & 1.000   & 0.962    & 0.992  & 0.984  & 0.992 & 0.992   & 0.866    & 0.984  & 1.000  & 0.988  & 0.994   & 1.000    & 1.000  \\
F17                    & non-hateful & 0.863  & 0.962 & 0.985   & 0.977    & 0.947  & 0.691  & 0.831 & 0.978   & 0.963    & 0.787  & 0.984  & 0.969 & 0.961   & 0.898    & 0.945  & 1.000  & 0.953  & 0.945   & 1.000    & 1.000  \\
F18                    & non-hateful & 0.611  & 0.788 & 0.442   & 0.982    & 0.292  & 0.410  & 0.689 & 0.213   & 0.910    & 0.008  & 0.068  & 0.239 & 0.000   & 0.761    & 0.000  & 0.991  & 0.929  & 0.549   & 1.000    & 0.982  \\
F19                    & non-hateful & 0.747  & 0.716 & 0.579   & 0.968    & 0.389  & 0.369  & 0.699 & 0.660   & 0.748    & 0.107  & 0.411  & 0.326 & 0.561   & 0.360    & 0.496  & 1.000  & 0.924  & 0.682   & 1.000    & 1.000  \\
F20                    & non-hateful & 1.000  & 0.900 & 1.000   & 1.000    & 1.000  & 0.600  & 0.600 & 1.000   & 1.000    & 0.800  & 0.800  & 0.700 & 0.700   & 1.000    & 0.700  & 1.000  & 0.969  & 1.000   & 1.000    & 1.000  \\
F21                    & non-hateful & 1.000  & 1.000 & 0.400   & 1.000    & 0.600  & 0.222  & 0.778 & 0.556   & 0.889    & 0.000  & 0.444  & 0.778 & 0.222   & 0.889    & 0.667  & 1.000  & 0.813  & 0.969   & 1.000    & 1.000  \\
F22                    & non-hateful & 0.778  & 1.000 & 0.667   & 1.000    & 0.667  & 0.400  & 0.600 & 0.800   & 1.000    & 0.100  & 0.167  & 0.833 & 0.000   & 0.667    & 0.167  & 1.000  & 1.000  & 1.000   & 1.000    & 1.000  \\
F23                    & hateful     & 0.473  & 0.087 & 0.793   & 0.020    & 0.660  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F24                    & hateful     & 0.351  & 0.145 & 0.634   & 0.015    & 0.664  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F25                    & hateful     & 0.457  & 0.371 & 0.836   & 0.000    & 0.784  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F26                    & hateful     & 0.513  & 0.026 & 0.704   & 0.017    & 0.757  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F27                    & hateful     & 0.414  & 0.080 & 0.816   & 0.011    & 0.713  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F32                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.630  & 0.225 & 0.732   & 0.174    & 0.674  & -      & -      & -       & -        & -      \\
F33                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.500  & 0.268 & 0.571   & 0.107    & 0.571  & -      & -      & -       & -        & -      \\
F34                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.596  & 0.404 & 0.750   & 0.038    & 0.769  & -      & -      & -       & -        & -      \\
\midrule
\multirow{3}{*}{Total} & non-hateful & 0.827  & 0.872 & 0.798   & 0.982    & 0.733  & 0.567  & 0.758 & 0.759   & 0.909    & 0.537  & 0.546  & 0.630 & 0.537   & 0.840    & 0.569  & 0.999  & 0.950  & 0.861   & 1.000    & 0.997  \\
                       & hateful     & 0.500  & 0.203 & 0.799   & 0.023    & 0.749  & 0.583  & 0.397 & 0.547   & 0.079    & 0.905  & 0.779  & 0.414 & 0.924   & 0.169    & 0.853  & 0.000  & 0.089  & 0.199   & 0.000    & 0.005  \\
                       & both  & 0.570  & 0.345 & 0.799   & 0.226    & 0.746  & 0.578  & 0.504 & 0.610   & 0.326    & 0.795  & 0.723  & 0.466 & 0.831   & 0.330    & 0.785  & 0.334  & 0.377  & 0.420   & 0.334    & 0.336 \\
\bottomrule
\end{tabular}
\caption{\textsf{SGHateCheck} functionalities accuracy for models fine-tuned in MultiSet (LL:LLaMA2, MB:mBert, MI:Mistral, SO:SEA-LION, SM: SeaLLM) and language. Notice how the bias is shown visually with greener non-hateful labels and redder hateful labels when 1) weaker models like SeaLLM are used, and 2) in Tamil, where training data is more scarce. }
\label{tab:annotation_functionality}
\end{table*}

==> model_bad.tex <==
\begin{tabular}{llllllll}
model   & training & hc bad & cn bad & en bad & ms bad & ta bad & zh bad \\
llama   & english  & 0      & 0      & 0      & 0      & 24     & 2      \\
sealion & english  & 3      & 1723   & 15     & 309    & 1979   & 1693   \\
sealion & seamulti & 0      & 0      & 0      & 0      & 1      & 0      \\  
\end{tabular}

==> tables/functionality-duplicate.tex <==
% \begin{table*}[]
% \small
% \centering
% \def\width{15mm}
% \def\arraystretch{1.5}
% \begin{tabular}{|p{1cm}|p{3cm}|p{1cm}}
% \hline
                                                              
% \end{tabular}
% \caption{Work in progress }
% \label{tab:functional_metrics}
% \end{table*}
\begin{sidewaystable*}
% \begin{table}
% \begin{adjustwidth}{-2em}{-2em}
\small
    \caption{SEA Hatecheck functionalities accuracy for each model (LL:LLaMA2, MB:mBert, MI:Mistral, SO:SEA-LION, SM: SeaLLM)  and language.}
\begin{tabular}{ll*{20}{c}}
\toprule
                       &             & \multicolumn{5}{c}{Singlish Accuracy}        & \multicolumn{5}{c}{Malay Accuracy}           & \multicolumn{5}{c}{Mandarin Accuracy}        & \multicolumn{5}{c}{Tamil Accuracy}            \\ \cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22}
F\#                    & Gold Label  & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM \\
\hline
F1                     & hateful     & 0.326  & 0.246 & 0.681   & 0.014    & 0.601  & 0.608  & 0.24  & 0.576   & 0.12     & 0.872  & 0.892  & 0.446 & 0.992   & 0.057    & 0.928  & 0.000      & 0.0227 & 0.037   & 0        & 0      \\
F2                     & hateful     & 0.398  & 0.096 & 0.831   & 0.000    & 0.771  & 0.620  & 0.463 & 0.639   & 0.046    & 0.954  & 0.794  & 0.431 & 1.000   & 0.157    & 0.971  & 0.000  & 0.056  & 0.112   & 0.000    & 0.000  \\
F3                     & hateful     & 0.427  & 0.183 & 0.779   & 0.000    & 0.740  & 0.508  & 0.308 & 0.523   & 0.015    & 0.954  & 0.877  & 0.352 & 0.984   & 0.074    & 0.926  & 0.000  & 0.056  & 0.126   & 0.000    & 0.000  \\
F4                     & hateful     & 0.492  & 0.150 & 0.734   & 0.017    & 0.671  & 0.507  & 0.271 & 0.243   & 0.100    & 0.650  & 0.566  & 0.184 & 0.846   & 0.279    & 0.640  & 0.000  & 0.056  & 0.175   & 0.000    & 0.040  \\
F4                     & hateful     & 0.519  & 0.130 & 0.878   & 0.000    & 0.702  & 0.470  & 0.289 & 0.417   & 0.104    & 0.922  & 0.755  & 0.230 & 0.942   & 0.137    & 0.921  & 0.000  & 0.057  & 0.100   & 0.000    & 0.000  \\
F5                     & hateful     & 0.703  & 0.464 & 0.964   & 0.007    & 0.935  & 0.647  & 0.489 & 0.619   & 0.079    & 0.978  & 0.829  & 0.464 & 0.950   & 0.214    & 0.929  & 0.000  & 0.131  & 0.238   & 0.000    & 0.000  \\
F7                     & hateful     & 0.600  & 0.000 & 0.500   & 0.000    & 0.500  & 0.556  & 0.556 & 0.333   & 0.000    & 0.778  & 1.000  & 0.400 & 0.800   & 0.000    & 0.600  & 0.000  & 0.100  & 0.000   & 0.000    & 0.000  \\
F8                     & hateful     & 0.579  & 0.214 & 0.793   & 0.007    & 0.779  & 0.629  & 0.500 & 0.536   & 0.064    & 0.886  & 0.928  & 0.667 & 1.000   & 0.232    & 0.877  & 0.000  & 0.044  & 0.106   & 0.000    & 0.000  \\
F9                     & non-hateful & 0.889  & 1.000 & 1.000   & 1.000    & 1.000  & 0.400  & 0.700 & 1.000   & 1.000    & 0.800  & 0.500  & 0.700 & 0.800   & 0.800    & 0.800  & 1.000  & 1.000  & 1.000   & 1.000    & 1.000  \\
F10                    & hateful     & 0.561  & 0.216 & 0.827   & 0.079    & 0.791  & 0.529  & 0.336 & 0.471   & 0.121    & 0.914  & 0.882  & 0.529 & 1.000   & 0.206    & 0.860  & 0.000  & 0.029  & 0.279   & 0.000    & 0.019  \\
F11                    & hateful     & 0.529  & 0.436 & 0.821   & 0.043    & 0.793  & 0.657  & 0.686 & 0.757   & 0.064    & 0.957  & 0.914  & 0.396 & 1.000   & 0.295    & 0.986  & 0.000  & 0.251  & 0.464   & 0.000    & 0.005  \\
F12                    & hateful     & 0.414  & 0.081 & 0.901   & 0.018    & 0.784  & 0.421  & 0.325 & 0.526   & 0.070    & 0.807  & 0.799  & 0.302 & 0.986   & 0.122    & 0.906  & 0.000  & 0.088  & 0.250   & 0.000    & 0.000  \\
F13                    & non-hateful & 0.871  & 0.823 & 0.895   & 0.992    & 0.887  & 0.608  & 0.672 & 0.856   & 0.904    & 0.688  & 0.555  & 0.609 & 0.609   & 0.875    & 0.703  & 1.000  & 0.934  & 0.766   & 1.000    & 0.993  \\
F14                    & hateful     & 0.574  & 0.156 & 0.803   & 0.049    & 0.787  & 0.677  & 0.339 & 0.710   & 0.097    & 0.992  & 0.835  & 0.729 & 1.000   & 0.256    & 0.970  & 0.000  & 0.152  & 0.296   & 0.000    & 0.000  \\
F15                    & hateful     & 0.722  & 0.357 & 0.930   & 0.087    & 0.957  & 0.703  & 0.461 & 0.578   & 0.070    & 0.992  & 0.949  & 0.594 & 0.993   & 0.130    & 0.971  & 0.000  & 0.052  & 0.156   & 0.000    & 0.000  \\
F16                    & non-hateful & 0.984  & 1.000 & 0.992   & 0.984    & 0.992  & 0.748  & 0.901 & 1.000   & 0.962    & 0.992  & 0.984  & 0.992 & 0.992   & 0.866    & 0.984  & 1.000  & 0.988  & 0.994   & 1.000    & 1.000  \\
F17                    & non-hateful & 0.863  & 0.962 & 0.985   & 0.977    & 0.947  & 0.691  & 0.831 & 0.978   & 0.963    & 0.787  & 0.984  & 0.969 & 0.961   & 0.898    & 0.945  & 1.000  & 0.953  & 0.945   & 1.000    & 1.000  \\
F18                    & non-hateful & 0.611  & 0.788 & 0.442   & 0.982    & 0.292  & 0.410  & 0.689 & 0.213   & 0.910    & 0.008  & 0.068  & 0.239 & 0.000   & 0.761    & 0.000  & 0.991  & 0.929  & 0.549   & 1.000    & 0.982  \\
F19                    & non-hateful & 0.747  & 0.716 & 0.579   & 0.968    & 0.389  & 0.369  & 0.699 & 0.660   & 0.748    & 0.107  & 0.411  & 0.326 & 0.561   & 0.360    & 0.496  & 1.000  & 0.924  & 0.682   & 1.000    & 1.000  \\
F20                    & non-hateful & 1.000  & 0.900 & 1.000   & 1.000    & 1.000  & 0.600  & 0.600 & 1.000   & 1.000    & 0.800  & 0.800  & 0.700 & 0.700   & 1.000    & 0.700  & 1.000  & 0.969  & 1.000   & 1.000    & 1.000  \\
F21                    & non-hateful & 1.000  & 1.000 & 0.400   & 1.000    & 0.600  & 0.222  & 0.778 & 0.556   & 0.889    & 0.000  & 0.444  & 0.778 & 0.222   & 0.889    & 0.667  & 1.000  & 0.813  & 0.969   & 1.000    & 1.000  \\
F22                    & non-hateful & 0.778  & 1.000 & 0.667   & 1.000    & 0.667  & 0.400  & 0.600 & 0.800   & 1.000    & 0.100  & 0.167  & 0.833 & 0.000   & 0.667    & 0.167  & 1.000  & 1.000  & 1.000   & 1.000    & 1.000  \\
F23                    & hateful     & 0.473  & 0.087 & 0.793   & 0.020    & 0.660  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F24                    & hateful     & 0.351  & 0.145 & 0.634   & 0.015    & 0.664  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F25                    & hateful     & 0.457  & 0.371 & 0.836   & 0.000    & 0.784  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F26                    & hateful     & 0.513  & 0.026 & 0.704   & 0.017    & 0.757  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F27                    & hateful     & 0.414  & 0.080 & 0.816   & 0.011    & 0.713  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F32                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.630  & 0.225 & 0.732   & 0.174    & 0.674  & -      & -      & -       & -        & -      \\
F33                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.500  & 0.268 & 0.571   & 0.107    & 0.571  & -      & -      & -       & -        & -      \\
F34                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.596  & 0.404 & 0.750   & 0.038    & 0.769  & -      & -      & -       & -        & -      \\
\midrule
\multirow{3}{*}{Total} & non-hateful & 0.827  & 0.872 & 0.798   & 0.982    & 0.733  & 0.567  & 0.758 & 0.759   & 0.909    & 0.537  & 0.546  & 0.630 & 0.537   & 0.840    & 0.569  & 0.999  & 0.950  & 0.861   & 1.000    & 0.997  \\
                       & hateful     & 0.500  & 0.203 & 0.799   & 0.023    & 0.749  & 0.583  & 0.397 & 0.547   & 0.079    & 0.905  & 0.779  & 0.414 & 0.924   & 0.169    & 0.853  & 0.000  & 0.089  & 0.199   & 0.000    & 0.005  \\
                       & both  & 0.570  & 0.345 & 0.799   & 0.226    & 0.746  & 0.578  & 0.504 & 0.610   & 0.326    & 0.795  & 0.723  & 0.466 & 0.831   & 0.330    & 0.785  & 0.334  & 0.377  & 0.420   & 0.334    & 0.336 \\
\bottomrule
\end{tabular}
% \end{adjustwidth}
% \end{table}
\end{sidewaystable*}

==> tables/functionality_table.tex <==
% \begin{table}
% \small
% \begin{tabular}{llRRRR}
% \toprule
%          F\#  & Label  & Sing.        & MS           & ZH       & TA           
% \\
% \hline
% F1                     & hateful  & 0.681   & 0.576  & 0.992   & 0.037     \\
% F2                     & hateful    & 0.831   & 0.639  & 1.000    & 0.112   \\
% F3                     & hateful    & 0.779   & 0.523   & 0.984   & 0.126   \\
% F4                     & hateful    & 0.878   & 0.417   & 0.942   & 0.100   \\
% F5                     & hateful    & 0.964   & 0.619   & 0.950   & 0.238   \\
% F7                     & hateful    & 0.500   & 0.333   & 0.800   & 0.000   \\
% F8                     & hateful    & 0.793   & 0.536   & 1.000   & 0.106   \\
% F9                     & non-hateful  & 1.000 & 1.000   & 0.800  & 1.000    \\
% F10                    & hateful     & 0.827   & 0.471    & 1.000   & 0.279    \\
% F11                    & hateful     & 0.821    & 0.757   & 1.000    & 0.464    \\
% F12                    & hateful     & 0.901    & 0.526    & 0.986    & 0.250     \\
% F13                    & non-hateful  & 0.895   & 0.856    & 0.609   & 0.766     \\
% F14                    & hateful      & 0.803   & 0.710    & 1.000     & 0.296    \\
% F15                    & hateful      & 0.930    & 0.578    & 0.993     & 0.156     \\
% F16                    & non-hateful  & 0.992    & 1.000    & 0.992    & 0.994   \\
% F17                    & non-hateful  & 0.985   & 0.978   & 0.961     & 0.945    \\
% F18                    & non-hateful  & 0.442   & 0.213   & 0.000     & 0.549     \\
% F19                    & non-hateful  & 0.579   & 0.660   & 0.561    & 0.682     \\
% F20                    & non-hateful  & 1.000   & 1.000   & 0.700    & 1.000    \\
% F21                    & non-hateful & 0.400   & 0.556   & 0.222     & 0.969    \\
% F22                    & non-hateful & 0.667    & 0.800    & 0.000     & 1.000     \\
% F23                    & hateful     & 0.793       & -          & -            & -            \\
% F24                    & hateful     & 0.634        & -         & -       & -           \\
% F25                    & hateful     & 0.836      & -      & -      & -          \\
% F26                    & hateful     & 0.704        & -      & -      & -        \\
% F27                    & hateful     & 0.816       & -       & -        & -      \\
% F32                    & hateful     & -     & -       & 0.732       & -         \\
% F33                    & hateful     & -      & -       & 0.571       & -      \\
% F34                    & hateful     & -      & -       & 0.750        & -      \\
% \midrule
% \multirow{3}{*}{Avg.} & non-hate  & 0.733    & 0.537  &      0.569    & 0.997  \\
%                        & hateful      & 0.799   & 0.547   & 0.924   & 0.199    \\
%                        & both   & 0.799   & 0.610   & 0.831   & 0.420  \\
% \bottomrule
% \end{tabular}
% \caption{\textsf{SGHateCheck} functionalities accuracy for models fine-tuned in MultiSet (LL:LLaMA2, MB:mBert, MI:Mistral, SO:SEA-LION, SM: SeaLLM) and language. Notice how the bias is shown visually with greener non-hateful labels and redder hateful labels when 1) weaker models like SeaLLM are used, and 2) in Tamil, where training data is more scarce. }
% \label{tab:annotation_functionality}
% \end{table}

\begin{sidewaystable*}
\small
\begin{tabular}{ll*{20}{R}}
\toprule
                       &             & \multicolumn{5}{c}{Singlish Accuracy}        & \multicolumn{5}{c}{Malay Accuracy}           & \multicolumn{5}{c}{Mandarin Accuracy}        & \multicolumn{5}{c}{Tamil Accuracy}            \\ \cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22}
F\#                    & Gold Label  & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM & LL & MB & MI & SO & SM \\
\hline
F1                     & hateful     & 0.326  & 0.246 & 0.681   & 0.014    & 0.601  & 0.608  & 0.24  & 0.576   & 0.120     & 0.872  & 0.892  & 0.446 & 0.992   & 0.057    & 0.928  & 0.000      & 0.022 & 0.037   & 0.000        & 0.000      \\
F2                     & hateful     & 0.398  & 0.096 & 0.831   & 0.000    & 0.771  & 0.620  & 0.463 & 0.639   & 0.046    & 0.954  & 0.794  & 0.431 & 1.000   & 0.157    & 0.971  & 0.000  & 0.056  & 0.112   & 0.000    & 0.000  \\
F3                     & hateful     & 0.427  & 0.183 & 0.779   & 0.000    & 0.740  & 0.508  & 0.308 & 0.523   & 0.015    & 0.954  & 0.877  & 0.352 & 0.984   & 0.074    & 0.926  & 0.000  & 0.056  & 0.126   & 0.000    & 0.000  \\
F4                     & hateful     & 0.492  & 0.150 & 0.734   & 0.017    & 0.671  & 0.507  & 0.271 & 0.243   & 0.100    & 0.650  & 0.566  & 0.184 & 0.846   & 0.279    & 0.640  & 0.000  & 0.056  & 0.175   & 0.000    & 0.040  \\
F4                     & hateful     & 0.519  & 0.130 & 0.878   & 0.000    & 0.702  & 0.470  & 0.289 & 0.417   & 0.104    & 0.922  & 0.755  & 0.230 & 0.942   & 0.137    & 0.921  & 0.000  & 0.057  & 0.100   & 0.000    & 0.000  \\
F5                     & hateful     & 0.703  & 0.464 & 0.964   & 0.007    & 0.935  & 0.647  & 0.489 & 0.619   & 0.079    & 0.978  & 0.829  & 0.464 & 0.950   & 0.214    & 0.929  & 0.000  & 0.131  & 0.238   & 0.000    & 0.000  \\
F7                     & hateful     & 0.600  & 0.000 & 0.500   & 0.000    & 0.500  & 0.556  & 0.556 & 0.333   & 0.000    & 0.778  & 1.000  & 0.400 & 0.800   & 0.000    & 0.600  & 0.000  & 0.100  & 0.000   & 0.000    & 0.000  \\
F8                     & hateful     & 0.579  & 0.214 & 0.793   & 0.007    & 0.779  & 0.629  & 0.500 & 0.536   & 0.064    & 0.886  & 0.928  & 0.667 & 1.000   & 0.232    & 0.877  & 0.000  & 0.044  & 0.106   & 0.000    & 0.000  \\
F9                     & non-hateful & 0.889  & 1.000 & 1.000   & 1.000    & 1.000  & 0.400  & 0.700 & 1.000   & 1.000    & 0.800  & 0.500  & 0.700 & 0.800   & 0.800    & 0.800  & 1.000  & 1.000  & 1.000   & 1.000    & 1.000  \\
F10                    & hateful     & 0.561  & 0.216 & 0.827   & 0.079    & 0.791  & 0.529  & 0.336 & 0.471   & 0.121    & 0.914  & 0.882  & 0.529 & 1.000   & 0.206    & 0.860  & 0.000  & 0.029  & 0.279   & 0.000    & 0.019  \\
F11                    & hateful     & 0.529  & 0.436 & 0.821   & 0.043    & 0.793  & 0.657  & 0.686 & 0.757   & 0.064    & 0.957  & 0.914  & 0.396 & 1.000   & 0.295    & 0.986  & 0.000  & 0.251  & 0.464   & 0.000    & 0.005  \\
F12                    & hateful     & 0.414  & 0.081 & 0.901   & 0.018    & 0.784  & 0.421  & 0.325 & 0.526   & 0.070    & 0.807  & 0.799  & 0.302 & 0.986   & 0.122    & 0.906  & 0.000  & 0.088  & 0.250   & 0.000    & 0.000  \\
F13                    & non-hateful & 0.871  & 0.823 & 0.895   & 0.992    & 0.887  & 0.608  & 0.672 & 0.856   & 0.904    & 0.688  & 0.555  & 0.609 & 0.609   & 0.875    & 0.703  & 1.000  & 0.934  & 0.766   & 1.000    & 0.993  \\
F14                    & hateful     & 0.574  & 0.156 & 0.803   & 0.049    & 0.787  & 0.677  & 0.339 & 0.710   & 0.097    & 0.992  & 0.835  & 0.729 & 1.000   & 0.256    & 0.970  & 0.000  & 0.152  & 0.296   & 0.000    & 0.000  \\
F15                    & hateful     & 0.722  & 0.357 & 0.930   & 0.087    & 0.957  & 0.703  & 0.461 & 0.578   & 0.070    & 0.992  & 0.949  & 0.594 & 0.993   & 0.130    & 0.971  & 0.000  & 0.052  & 0.156   & 0.000    & 0.000  \\
F16                    & non-hateful & 0.984  & 1.000 & 0.992   & 0.984    & 0.992  & 0.748  & 0.901 & 1.000   & 0.962    & 0.992  & 0.984  & 0.992 & 0.992   & 0.866    & 0.984  & 1.000  & 0.988  & 0.994   & 1.000    & 1.000  \\
F17                    & non-hateful & 0.863  & 0.962 & 0.985   & 0.977    & 0.947  & 0.691  & 0.831 & 0.978   & 0.963    & 0.787  & 0.984  & 0.969 & 0.961   & 0.898    & 0.945  & 1.000  & 0.953  & 0.945   & 1.000    & 1.000  \\
F18                    & non-hateful & 0.611  & 0.788 & 0.442   & 0.982    & 0.292  & 0.410  & 0.689 & 0.213   & 0.910    & 0.008  & 0.068  & 0.239 & 0.000   & 0.761    & 0.000  & 0.991  & 0.929  & 0.549   & 1.000    & 0.982  \\
F19                    & non-hateful & 0.747  & 0.716 & 0.579   & 0.968    & 0.389  & 0.369  & 0.699 & 0.660   & 0.748    & 0.107  & 0.411  & 0.326 & 0.561   & 0.360    & 0.496  & 1.000  & 0.924  & 0.682   & 1.000    & 1.000  \\
F20                    & non-hateful & 1.000  & 0.900 & 1.000   & 1.000    & 1.000  & 0.600  & 0.600 & 1.000   & 1.000    & 0.800  & 0.800  & 0.700 & 0.700   & 1.000    & 0.700  & 1.000  & 0.969  & 1.000   & 1.000    & 1.000  \\
F21                    & non-hateful & 1.000  & 1.000 & 0.400   & 1.000    & 0.600  & 0.222  & 0.778 & 0.556   & 0.889    & 0.000  & 0.444  & 0.778 & 0.222   & 0.889    & 0.667  & 1.000  & 0.813  & 0.969   & 1.000    & 1.000  \\
F22                    & non-hateful & 0.778  & 1.000 & 0.667   & 1.000    & 0.667  & 0.400  & 0.600 & 0.800   & 1.000    & 0.100  & 0.167  & 0.833 & 0.000   & 0.667    & 0.167  & 1.000  & 1.000  & 1.000   & 1.000    & 1.000  \\
F23                    & hateful     & 0.473  & 0.087 & 0.793   & 0.020    & 0.660  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F24                    & hateful     & 0.351  & 0.145 & 0.634   & 0.015    & 0.664  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F25                    & hateful     & 0.457  & 0.371 & 0.836   & 0.000    & 0.784  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F26                    & hateful     & 0.513  & 0.026 & 0.704   & 0.017    & 0.757  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F27                    & hateful     & 0.414  & 0.080 & 0.816   & 0.011    & 0.713  & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & -      & -      & -       & -        & -      \\
F32                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.630  & 0.225 & 0.732   & 0.174    & 0.674  & -      & -      & -       & -        & -      \\
F33                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.500  & 0.268 & 0.571   & 0.107    & 0.571  & -      & -      & -       & -        & -      \\
F34                    & hateful     & -      & -     & -       & -        & -      & -      & -     & -       & -        & -      & 0.596  & 0.404 & 0.750   & 0.038    & 0.769  & -      & -      & -       & -        & -      \\
\midrule
\multirow{3}{*}{Total} & non-hateful & 0.827  & 0.872 & 0.798   & 0.982    & 0.733  & 0.567  & 0.758 & 0.759   & 0.909    & 0.537  & 0.546  & 0.630 & 0.537   & 0.840    & 0.569  & 0.999  & 0.950  & 0.861   & 1.000    & 0.997  \\
                       & hateful     & 0.500  & 0.203 & 0.799   & 0.023    & 0.749  & 0.583  & 0.397 & 0.547   & 0.079    & 0.905  & 0.779  & 0.414 & 0.924   & 0.169    & 0.853  & 0.000  & 0.089  & 0.199   & 0.000    & 0.005  \\
                       & both  & 0.570  & 0.345 & 0.799   & 0.226    & 0.746  & 0.578  & 0.504 & 0.610   & 0.326    & 0.795  & 0.723  & 0.466 & 0.831   & 0.330    & 0.785  & 0.334  & 0.377  & 0.420   & 0.334    & 0.336 \\
\bottomrule
\end{tabular}
\caption{\textsf{SGHateCheck} functionalities accuracy for models fine-tuned in MultiSet (LL:LLaMA2, MB:mBert, MI:Mistral, SO:SEA-LION, SM: SeaLLM) and language. Notice how the bias is shown visually with greener non-hateful labels and redder hateful labels when 1) weaker models like SeaLLM are used, and 2) in Tamil, where training data is more scarce. }
\label{tab:annotation_functionality}
\end{sidewaystable*}

==> tables/heldout_table.tex <==
\begin{table}[]
\begin{tabular}{llllllll}
                          &                            &            & Llama       & mBert       & Mistral     & SEA-LION    & SeaLLM      \\
\multirow{3}{*}{F1}       & English                    & hatexplain & 0.722513089 & 0.744715447 & 0.756159728 & 0.064516129 & 0.72489083  \\
                          & \multirow{2}{*}{SeaMulti1} & hatexplain & 0.728353141 & 0.752902156 & 0.703636364 & 0.192       & 0.657065707 \\
                          &                            & COLD       & 0.719096334 & 0.781223084 & 0.763375381 & 0.378189095 & 0.749403341 \\
\multirow{3}{*}{Accuracy} & English                    & hatexplain & 0.834719335 & 0.836798337 & 0.850831601 & 0.667188315 & 0.836278586 \\
                          & \multirow{2}{*}{SeaMulti1} & hatexplain & 0.833679834 & 0.845114345 & 0.830561331 & 0.685031185 & 0.801975052 \\
                          &                            & COLD       & 0.797294759 & 0.80913019  & 0.795603983 & 0.532882375 & 0.783017096
\end{tabular}
\end{table}
